Personalized Differential Privacy for Ridge Regression

The increased application of machine learning (ML) in sensitive domains requires protecting the training data through privacy frameworks, such as differential privacy (DP). DP requires to specify a uniform privacy level $\varepsilon$ that expresses the maximum privacy loss that each data point in the entire dataset is willing to tolerate. Yet, in practice, different data points often have different privacy requirements. Having to set one uniform privacy level is usually too restrictive, often forcing a learner to guarantee the stringent privacy requirement, at a large cost to accuracy. To overcome this limitation, we introduce our novel Personalized-DP Output Perturbation method (PDP-OP) that enables to train Ridge regression models with individual per data point privacy levels. We provide rigorous privacy proofs for our PDP-OP as well as accuracy guarantees for the resulting model. This work is the first to provide such theoretical accuracy guarantees when it comes to personalized DP in machine learning, whereas previous work only provided empirical evaluations. We empirically evaluate PDP-OP on synthetic and real datasets and with diverse privacy distributions. We show that by enabling each data point to specify their own privacy requirement, we can significantly improve the privacy-accuracy trade-offs in DP. We also show that PDP-OP outperforms the personalized privacy techniques of Jorgensen et al. (2015).

==> privacy_data_corr.tex <==
In certain sensitive applications, an individual's choice of privacy budget can reflect some sensitive information. 
Imagine a medical context with a dataset that consists of individuals that do and individuals that do not have a rare disease.
The latter ones might prefer higher privacy protection to hide their condition. If an attacker with access to the trained model was able to deduce the individual's privacy budget, they might, in turn, be able to draw conclusions on the individual's medical state. This provides a point of attack towards our privacy guarantees. 

We note, however, that deducing privacy budgets is generally a hard problem, alleviating our concerns when it comes to data--privacy budget correlations. Theoretical results from ML, e.g.,~\cite{gilbert2018property}, have shown that one cannot currently perform sample-efficient black-box audits to determine the privacy-budget of a trained model. 
